Distributed non-negative RESCAL with Automatic Model Selection for Exascale Data

With the boom in the development of computer hardware and software, social media, IoT platforms, and communications, there has been an exponential growth in the volume of data produced around the world. Among these data, relational datasets are growing in popularity as they provide unique insights regarding the evolution of communities and their interactions. Relational datasets are naturally non-negative, sparse, and extra-large. Relational data usually contain triples, (subject, relation, object), and are represented as graphs/multigraphs, called knowledge graphs, which need to be embedded into a low-dimensional dense vector space. Among various embedding models, RESCAL allows learning of relational data to extract the posterior distributions over the latent variables and to make predictions of missing relations. However, RESCAL is computationally demanding and requires a fast and distributed implementation to analyze extra-large real-world datasets. Here we introduce a distributed non-negative RESCAL algorithm for heterogeneous CPU/GPU architectures with automatic selection of the number of latent communities (model selection), called pyDRESCALk. We demonstrate the correctness of pyDRESCALk with real-world and large synthetic tensors, and the efficacy showing near-linear scaling that concurs with the theoretical complexities. Finally, pyDRESCALk determines the number of latent communities in an 11-terabyte dense and 9-exabyte sparse synthetic tensor.

==> Complexity.tex <==
\subsection{Complexity of distributed Rescal}

The experiments were performed on the HPC cluster Grizzly, located at Los Alamos National Laboratory (LANL). It uses Intel OmniPath interconnect having a fat tree topology. Hence, we assume a fully connected network for calculating all our communication complexities. 

%\subsubsection{Communication model}
%We used the latency, bandwidth, and computation model of distributed memory parallel computation to analyze the algorithms discussed in this paper\cite{chan2007collective}. In this model, $\alpha$ denotes the latency or start-up times, $\beta$ the per data item transmission time, and $\gamma$ the time to perform an arithmetic operation. The communication between two processors is modeled as messages sent across a bidirectional link, so the resulting cost of transmitting $n$ data items is described as $\alpha + n\beta$. The performance of an algorithm can be predicted in terms of the number of data items it communicates as well as the number of flops it performs. The possibilities of overlapping computation and communication have been ignored for simplicity. 

%\subsubsection{MPI Collectives}
%MPI provides an interface for collective communication which involves participation of all processes involved in the communicator. The MPI collectives include broadcast, gather, scatter and reduce. We have used, all-reduce, reduce-scatter and all-gather in our algorithms. For gather and scatter operations, the root node sends or receives $\frac{p-1}{p}n$ items with a cost of $\frac{p-1}{p}n\beta$~\cite{chan2007collective}. For reduce, the root node sends or receives $n$ items with cost of $n\beta$. Each $p$ processors owns a data of size $\frac{n}{p}$ and a copy of the entire data size $n$ at the start and end of an all-gather collective respectively. The cost of an all-gather is $\alpha . log p + \beta\frac{p-1}{p}n$. 
%For a reduce-scatter, each processor owns a copy of the entire data size $n$ at the start and a subset of sum over all the data having size $\frac{n}{p}$ after a reduce-scatter. The cost of a reduce-scatter is $\alpha . log p + {\beta+\gamma}\frac{p-1}{p}n$. 
%For an all-reduce, each processor owns a data of size n at the start and end of the all-reduce operation. The cost of an all-reduce is $2\alpha . log p + {2\beta+\gamma}\frac{p-1}{p}n$. The costs of each of the collectives are zero when p=1.


\begin{table*}[]
    \centering
    \begin{tabular}{c|ccc}
         algorithm & Communication complexity& Computation Complexity/Flops & Memory  \\
         \hline
         %Broadcast & $\ceil*{\log_2(p)} \alpha$ & $n\beta$ & --\\
         DnRESCAL(Dense) & $(2\alpha log(\sqrt{p}) + 2\beta k^2) + (2\alpha log(\sqrt{p}) + 2\beta\frac{\sqrt{p}-1}{p}kn)$ & $2mn^2k + (3m+2)nk^2 + nk + mk^3$ & $\frac{mn^2}{p}+(mk+\frac{2n}{\sqrt p})kr+(r+1)2rk$\\

         DnRESCAL(Sparse) & $(2\alpha log(\sqrt{p}) + 2\beta k^2) + (2\alpha log(\sqrt{p}) + 2\beta\frac{\sqrt{p}-1}{p}kn)$ & $4mn^2\delta k + (3m+2)nk^2 + nk + mk^3$  & $\frac{(m\delta)^2}{p}+(mk+\frac{2n}{\sqrt p})kr+(r+1)2rk$ \\
         DnRESCALk(Dense) & $\frac{mnk_u^2r}{\sqrt p}+\frac{r^2k_u^3n}{\sqrt p}+k_u^3r^2 \sqrt p+k_u^4r^2$ & $k_u^2r(k_ur+\sqrt{mn/\sqrt p})$ & - \\
    \end{tabular}
    \caption{Caption}
    \label{tab:complexity_chart}
\end{table*}

\subsubsection{Communication Complexity}
In this section, we compute communication complexities for the 2D distributed scheme of multiplicative updates used in our RESCAL implementation.
There are 4 occurences of reduce in our algorithm which is looped over m dimension of tensor. Thus, the cost for reduce for our algorithm is $(m+1)(log(\sqrt{p})k^2) + 2m(log(\sqrt{p})\frac{kn}{\sqrt{p}})$.
%Also, there are 2 occurences of broadcast which corresponds to $(m+1)(log(\sqrt{p})\frac{kn}{\sqrt{p}})$.
Therefore, the total communication complexity for Rescal algorithm with multiplicative update is $(log(\sqrt{p})k^2) + (log(\sqrt{p})\frac{kn}{\sqrt{p}})$. The communication complexity is same for both dense and sparse data.

\subsubsection{Computational Complexity}
The computational complexity for calculating ${A}^T{A}$ for both dense and sparse is $nk^2$. However, the computational complexity for calculating $\ten{X}{A}$ or $\ten{X}^T{A}$ is $mn^2k$ for dense \ten{X} and $2mn^2\delta k$ for sparse, where $\delta$ is the density. Similarly, the total computational complexity for our rescal algorithm is $2mn^2k + (3m+2)nk^2 + nk + mk^3$ for dense $\ten{X}$ and $4mn^2\delta k + (3m+2)nk^2 + nk + mk^3$ for sparse $\ten{X}$.



==> Speedup_Calculation.tex <==
\subsection{Speedup}

The speedup is calculated differently in strong and weak scaling experiments. In case of strong scaling experiment where the problem size is kept same and the number of processing elements are increased, speedup is calculated as a ratio of the time taken by sequential algorithm (i.e. running the algorithm on 1 processing element) over the time taken by the parallel algorithm (i.e. running on p processing elements). The efficiency is then computed as speedup by the number of processors. 

However, in weak scaling experiment, we cannot use the same formula as discussed above since our problem size is not kept same with increasing processors. Thus, the efficiency is calculated as $\frac{Total computational Time}{Total Time}$ and speedup is $p * Efficiency$.
